FireLedger: A High Throughput Blockchain Consensus Protocol

Blockchains are distributed secure ledgers to which transactions are issued continuously and each block of transactions is tightly coupled to its predecessors. Permissioned blockchains place special emphasis on transactions throughput. In this paper we present FireLedger, which leverages the iterative nature of blockchains in order to improve their throughput in optimistic execution scenarios. FireLedger trades latency for throughput in the sense that in FireLedger the last f + 1 blocks of each node's blockchain are considered tentative, i.e., they may be rescinded in case one of the last f + 1 blocks proposers was Byzantine. Yet, when optimistic assumptions are met, a new block is decided in each communication step, which consists of a proposer that sends only its proposal and all other participants are sending a single bit each. Our performance study demonstrates that in a single Amazon data-center, FireLedger running on 10 mid-range Amazon nodes obtains a throughput of up to 160K transactions per second for (typical Bitcoin size) 512 bytes transactions. In a 10 nodes Amazon geo-distributed setting with 512 bytes transactions, FireLedger obtains a throughput of 30K tps. Moreover, on higher end Amazon machines, FireLedger obtains $20%-600%$ better throughput than state of the art protocols like HotStuff and BFT-SMaRt, depending on the exact configuration.

==> sections/preliminaries2.tex <==
\section{Preliminaries}
\label{sec:prelim}

\subsection{System Model}
We consider an asynchronous fully connected environment consisting of $n$ nodes out of which at most $f < \frac{n}{3}$ may incur Byzantine failures~\cite{AW98,Raynal2018book}.
\iftoggle{FV}{
Asynchronous means that no upper bound on the messages' transfer delays exists and nodes have no access to a global clock.
While nodes may have access to local clocks, these clocks might not be synchronized with each other and may advance at different rates.}
{}
Fully connected means that any two nodes are connected via a reliable link.
Reliable means that a link does not lose, modify or duplicate a sent message.
Notice that unreliable fair lossy links can be transformed into reliable ones using sequence numbering, retransmissions, and error detection codes~\cite{Coding-Theory-Book}.
A Byzantine failure means that a node might deviate arbitrarily w.r.t. its protocol code including, e.g., sending arbitrary messages, sending messages with different values to different nodes, or failing to send any or all messages.
Yet, we assume that nodes cannot impersonate each other.
A node suffering from a Byzantine failure at any point during its operation is called \emph{Byzantine}; otherwise, it is said to be \emph{correct}.

\iftoggle{FV}{
Following the FLP result~\cite{Fischer1985}, consensus is unsolvable in a truly asynchronous system.
We circumvent FLP by enriching the system with the $\bDiamond \mathit{Synch}$  assumption~\cite{Bouzid2015}.
$\bDiamond \mathit{Synch}$ means that after an unknown time $\tau$ there is an unknown upper bound $\delta$ on a message's transfer delay.
}
{In order to circumvent the FLP result~\cite{Fischer1985}, we enrich the system with the $\bDiamond \mathit{Synch}$  assumption~\cite{Bouzid2015}.
That is, after an unknown time $\tau$ there is an unknown upper bound $\delta$ on a message's transfer delay.
}
As in most Byzantine fault tolerance works~\cite{Guerraoui2010,Castro1999,Kotla2007}, $\bDiamond \mathit{Synch}$  is only needed to ensure liveness, meaning that even under severe network delays safety is never violated.
Finally, a node may sign a message by an unforgeable signature.
We denote the signature of node $p$ on message $m$ by $sig_p(m)$.
The implementation of the signature mechanism is done by a well known cryptographic technique, such as symmetric ciphers~\cite{Ebrahim2014}, RSA~\cite{Rivest1978} or an elliptic curves digital signature (ECDS)~\cite{Johnson2001}.
	
\subsection{Underlying Protocols}
Solutions to the following fundamental distributed computing problems serve as building blocks for \PROTNAME.

\paragraph*{Reliable Broadcast (RB)}
The reliable broadcast abstraction~\cite{Bracha1987} (denoted \textbf{RB-Broadcast}) ensures reliable message delivery in the presence of Byzantine failures.
To utilize \textbf{RB-Broadcast} nodes may invoke two methods: \emph{RB-broadcast} and \emph{RB-deliver}.
A correct node that wishes to broadcast a message $m$ invokes \emph{RB-broadcast(m)} while a node that expects to receive a message invokes \emph{RB-deliver}.
By a slight abuse of notation, we denote \emph{RB-deliver(m)} the fact that an invocation of \emph{RB-deliver} returned the message $m$ and say that the invoking process has RB-delivered $m$.
The \textbf{RB-Broadcast} abstraction satisfies the following properties:
\iftoggle{FV}{
\iftoggle{MYACM}{
	\begin{description}
}{	
	\begin{LaTeXdescription}
}
		\item[RB-Validity:] If a correct node has RB-delivered a message $m$ from a correct node $p$, then $p$ has invoked \emph{RB-broadcast(m)}.
		%\item \emph{RB-Unicity:} For a given unique message $m$, every correct node \emph{RB-delivers} $m$ at most once.
		\item[RB-Agreement:] If a correct node \emph{RB-delivers} a message $m$, then all correct nodes eventually \emph{RB-deliver} $m$.
		\item[RB-Termination:] If a correct node invokes \emph{RB-broadcast(m)}, then all correct nodes eventually \emph{RB-deliver} $m$.
	\iftoggle{MYACM}{
	\end{description}
	}{	
	\end{LaTeXdescription}
}
}{\\
	\noindent\textbf{*~RB-Validity:} If a correct node has RB-delivered a message $m$ from a correct node $p$, then $p$ has invoked \emph{RB-broadcast(m)}.\\
	%\item \emph{RB-Unicity:} For a given unique message $m$, every correct node \emph{RB-delivers} $m$ at most once.
	\noindent\textbf{*~RB-Agreement:} If a correct node \emph{RB-delivers} a message $m$, then all correct nodes eventually \emph{RB-deliver} $m$.\\
	\noindent\textbf{*~RB-Termination:} If a correct node invokes \emph{RB-broadcast(m)}, then all correct nodes eventually \emph{RB-deliver} $m$.
}

\paragraph*{Atomic Broadcast (AB)}
\iftoggle{FV}{
The atomic broadcast abstraction~\cite{Cristian95} is more restrictive than \textbf{RB-Broadcast} in the sense that in addition to the \emph{RB-Broadcast} properties it requires the \emph{Order} property as well.
}
{
	Atomic broadcast~\cite{Cristian95} adds the following \emph{Order} property to \textbf{RB-Broadcast}.
}
\iftoggle{FV}{
\iftoggle{MYACM}{
	\begin{description}
	}{	
	\begin{LaTeXdescription}
}
		\item[Atomic-Order:] All messages delivered by correct nodes are delivered in the same order by all correct nodes.
	\iftoggle{MYACM}{
	\end{description}
}{	
	\end{LaTeXdescription}
}
}{
\\
\noindent\textbf{*~Atomic-Order:} Messages delivered by correct nodes are delivered in the same order by all correct nodes.
}
\begin{comment}
\iftoggle{FV}{

\paragraph*{Multi-value Byzantine Consensus}
Most implementations of atomic broadcast rely on consensus protocols as sub-routines.
In our context, \emph{Multi-value Byzantine Consensus} (MVC)~\cite{Lamport1982} is a variant of the consensus problem in which a set of nodes, each potentially proposing its own value, must decide the same value in a decentralized network despite the presence of Byzantine failures.
A solution to the MVC problem satisfies the following properties~\cite{Dwork1988}:
	%source
\iftoggle{MYACM}{
	\begin{description}
	}{	
		\begin{LaTeXdescription}
		}
		\item[MVC-Validity:] If all correct nodes have proposed the same value $v$, then $v$ must be decided.
		\item[MVC-Agreement:] No two correct nodes decide differently.
		\item[MVC-Termination:] Each correct node eventually decides.
	\iftoggle{MYACM}{
\end{description}
}{	
\end{LaTeXdescription}
}
Notice that according to \textbf{MVC-Validity}, any decision is valid when not all correct nodes propose the same value.
Hence, it is not helpful when the system begins in a non agreement state, which is common in real systems.
To that end, an extended validity property was suggested in~\cite{Correia2005} and is composed of three sub-properties:
\iftoggle{MYACM}{
	\begin{description}
	}{	
		\begin{LaTeXdescription}
		}
		\item[MVC1-Validity:] If all correct nodes have proposed the same value $v$, then $v$ must be decided.
		\item[MVC2-Validity:] A decided value $v$ was proposed by some node or $v=nil$.
		\item[MVC3-Validity:] No correct node decides a value that was proposed by only faulty nodes.
	\iftoggle{MYACM}{
\end{description}
}{	
\end{LaTeXdescription}
}
This validity property defines that if no correct node has suggested $v$, then $v$ cannot be decided.
This definition states precisely what is the set of valid values in any possible run of the algorithm.

\paragraph*{(Optimistic) Binary Byzantine Consensus}
The \emph{Binary Byzantine Consensus} (BBC) is the simplest variant of MVC in which only two values are possible.
The \textbf{MVC-Validity}, \textbf{MVC-Agreement}, and \textbf{MVC-Termination} properties naturally translate to their corresponding \textbf{BBC-Validity}, \textbf{BBC-Agreement}, and \textbf{BBC-Termination} properties.
Interestingly, BBC cannot be solved in a weaker model than MVC.
However, as only two values are possible, an \emph{Optimistic BBC} (OBBC) is capable of achieving an agreement in a single communication step if a predefined set of conditions is met \cite{Friedman:2005, Mosfaoui:2015}.

}{
\end{comment}
\paragraph*{(Optimistic) Binary Byzantine Consensus}
\emph{Binary Byzantine Consensus} (BBC) is the simplest variant of \emph{BFT Consensus}~\cite{Lamport1982} in which only two values are possible. 
A solution to the BBC problem satisfies the following properties~\cite{Correia2005, Dwork1988}:
\iftoggle{FV}{
	\iftoggle{MYACM}{
		\begin{description}
	}{	
	\begin{LaTeXdescription}
	}
		\item[BBC-Validity:] If all correct nodes have proposed the same value $v$, then $v$ must be decided.
		\item[BBC-Agreement:] No two correct nodes decide differently.
		\item[BBC-Termination:] Each correct node eventually decides.
	\iftoggle{MYACM}{
	\end{description}
	}{	
	\end{LaTeXdescription}
}
}{
\\
\noindent\textbf{*~BBC-Validity:} If all correct nodes have proposed the same value $v$, then $v$ must be decided.\\
\noindent\textbf{*~BBC-Agreement:} No two correct nodes decide differently.\\
\noindent\textbf{*~BBC-Termination:} Each correct node eventually decides.
%\begin{LaTeXdescription}
	%\item[BBC-Validity:] If all correct nodes have proposed the same value $v$, then $v$ must be decided.
	%\item[BBC-Agreement:] No two correct nodes decide differently.
	%\item[BBC-Termination:] Each correct node eventually decides.
%\end{LaTeXdescription}
}
As there are only two possible values in BBC, an \emph{Optimistic BBC} (OBBC) is capable of achieving an agreement in a single communication step if a predefined set of favorable conditions are met~\cite{YRP2,Friedman:2005,Mosfaoui:2015}.
%}
%\begin{comment}
%\subsection{Leveraging Blockchain's Iterativity}
%Blockchain algorithms require an external validity mechanism as sometimes even Byzantine nodes may propose legal values (or %blocks)~\cite{Luu:2016}.
%Therefore, the validity of a value may be defined by an external predefined method.
%The \emph{Validity Predicate-based Byzantine Consensus} (VPBC)~\cite{CKPS01,Crain2017} abstraction captures this observation by defining the %following validity property:
%\iftoggle{FV}{
%\iftoggle{MYACM}{
%	\begin{description}
%	}{	
%		\begin{LaTeXdescription}
%		}
%	\item[VPBC-Validity:] A decided value satisfies an external predefined \textsc{valid} method.
%	\iftoggle{MYACM}{
%\end{description}
%}{	
%\end{LaTeXdescription}
%}
%}{
%\\
%\noindent\textbf{*~VPBC-Validity:} A decided value satisfies an external predefined \textsc{valid} method.\\
%}
%\textbf{VPBC-Agreement} and \textbf{VPBC-Termination} are the same as their MVC/BBC counterparts.
%That is,  VPBC  generalizes the classical definition of MVC.

%\paragraph*{Iterative Validity Predicate-based Consensus}
%In order to leverage the iterative nature of blockchains, we define a weaker model than \emph{VPBC} in which we denote each iteration with a %round number $r$.
%Next, we define the following per round notions:
%\iftoggle{MYACM}{
%	\begin{description}
%	}{	
%		\begin{LaTeXdescription}
%		}
%	\item[Tentative decision:] A decision of the protocol at a given node and round that might still be changed.
%	\item[Definite decision:] A decision of the protocol at a given node and round that will never change.
%	\item[\boldmath{$v_{p}^{r}$}:] A value that was decided or received by $p$ in round $r$ of the protocol. $v^r$ denotes a value that was decided or received by some node in round $r$.
%	\item[\boldmath{$d(v_p^r)$}:] Let $r'$ be the current round of the protocol that node $p$ runs. For a given $v_{p}^{r}$ (possible tentative), we denote its \emph{depth} as $d(v_{p}^{r}) = r' - r$.
%	\iftoggle{MYACM}{
%\end{description}
%}{	
%\end{LaTeXdescription}
%}

%\begin{table}
%\centering
%\begin{tabu} to 1 \textwidth {|| m{2cm} | m{5cm} ||}
%\hline
%\emph{Tentative decision} & \makecell{A decision of the protocol\\at a given node and round that might still be changed}\\
%\hline \emph{Definite decision} & \makecell{A decision of the protocol\\at a given node and round that will never be changed}\\
%\hline $v_{p}^{r}$ & \makecell{A value that was decided or received by $p$ in round $r$ of the protocol.\\$v^r$ denotes a value that was %decided or received by some node in round $r$} \\
%\hline
%$d(v_p^r)$ & \makecell{Let $r'$ be the current round of the protocol that node $p$ runs.\\For a given $v_{p}^{r}$ (possible tentative), we denote its \emph{depth} as $d(v_{p}^{r}) = r' - r$}\\
%\hline
%\end{tabu}
%\end{table}


%Let \textsc{valid} be a predefined method as in VPBC and let $\rho$ be a predefined fixed constant.
%The $\rho$\emph{-Iterative Validity Predicate-based Consensus} (IVPC($\rho$)) abstraction defines the following properties:
%\iftoggle{FV}{
%\iftoggle{MYACM}{
%	\begin{description}
%	}{	
%		\begin{LaTeXdescription}
%		}
%	\item[IVPC-Validity:] A decided (possible tentative) value $v$ satisfies the \textsc{valid} method.
%	\item[IVPC-Agreement:] For any two correct nodes $p,q$, let $v_p^r, v_q^r$ be their decided value in round $r$. If $d(v_p^r), d(v_q^r) > \rho$ then $v_p^r=v_q^r$.
%	\item[IVPC-Termination(1):] Every round eventually terminates.
%	\item[IVPC-Termination(2):] In every round $r' > r + \rho$, $v_p^r$ is definite.
%	\iftoggle{MYACM}{
%\end{description}
%}{	
%\end{LaTeXdescription}
%}
%}{
%\\
%\noindent\textbf{*~IVPC-Validity:} A decided (possible tentative) value $v$ satisfies the \textsc{valid} method.\\
%\noindent\textbf{*~IVPC-Agreement:} For any two correct nodes $p,q$, let $v_p^r, v_q^r$ be their decided value in round $r$. If $d(v_p^r), d(v_q^r) > \rho$ then $v_p^r=v_q^r$.\\
%\noindent\textbf{*~IVPC-Termination(1):} Every round eventually terminates.\\
%\noindent\textbf{*~IVPC-Termination(2):} In every round $r' > r + \rho$, $v_p^r$ is definite.\\
%}
%IVPC guarantees the VPBC's properties only for decisions at depth greater than $\rho$.
%With blockchains, as every block contains an authentication data regarding its predecessors, it provides a glimpse to its creator history.
%This additional information may assist in detecting failures without the necessity of sending additional information.
%In addition, blocks are continuously added to the chain.
%Thus, a block eventually becomes deep enough such that it satisfies the standard VPBC properties.
%Let us note that the IVPC-Agreement property is similar to the notion of \emph{common prefix} in~\cite{Garay15}.

%In a blockchain setting, \emph{clients} of the system submit \emph{transactions} to the nodes, and the decisions values are blocks, each consisting of zero or more transactions previously submitted by clients.
%In case the \textsc{valid} method may accept empty blocks, we would like to prevent trivial implementations in which every node locally generates empty blocks continuously.
%Obviously, the throughput of such a protocol would be $0$, and thus it would be considered useless.
%Yet, in order to prove that a protocol does not unintentionally suffer from such a behavior even under Byzantine failures we add the following requirement:
%\iftoggle{FV}{
%\iftoggle{MYACM}{
%	\begin{description}
%	}{	
%		\begin{LaTeXdescription}
%		}
%	\item[Non-Triviality:] If clients repeatedly submit transactions to the system, then the nodes repeatedly decide definitively non-empty blocks. 
%	\iftoggle{MYACM}{
%\end{description}
%}{	
%\end{LaTeXdescription}
%}
%}{
%\\
%\noindent\textbf{*~Non-Triviality:} If clients repeatedly submit transactions to the system, then the nodes repeatedly decide definitively non-empty blocks. 

%}



==> sections/toy.tex <==
\iftoggle{Annon}{
\section{The \PROTNAME{} Protocol}
}
{
\section{\PROTNAME -- a Total ordering Optimistic sYstem}
}
\label{sec:toy}

\iftoggle{FV}{
\PROTNAME{} implements the IVPC($\rho$) abstraction with $\rho = f + 1$.
This section focuses on the algorithmic aspects of \PROTNAME{} and its correctness, while actual implementation considerations and performance are discussed in Section~\ref{sec:impl} below.
}{
}


\subsection{Overview}
\label{sec:toy-overview}
\begin{comment}
We now present \PROTNAME, a Total ordering Optimistic sYstem, targeting blockchains.
\PROTNAME{} implements the IVPC($\rho$) abstraction with $\rho = f + 1$.
It performs a single communication step per round in the fault-free and synchronized case.
We discuss \PROTNAME's performances in details as well as its strengths and weaknesses in Section~\ref{sec:eval}.
\end{comment}

\iftoggle{FV}{
}{
We now present \PROTNAME, which implements the IVPC($\rho$) abstraction with $\rho = f + 1$.
}
In the fault-free synchronized case, \PROTNAME{} decides on a new block in each communication step.
Further, in each such step a single proposer sends its proposed block and all other nodes only send a single bit (plus headers).
In order to achieve these goals, \PROTNAME{} runs speculatively assuming that there are no failures and the network is synchronized.
To that end, it employs a rotating proposer paradigm in which the proposer of each round advances in a cyclic manner.
In each round, the proposer simply broadcasts its proposed block.

Obviously, sometimes the optimistic assumptions do not hold.
\PROTNAME{} separates between how it recovers from benign failures which cause one or more nodes to miss a message vs. how it handles non-benign failures that may cause different nodes to hold a diverging suffix of the blockchain.
Yet, unlike most consensus based protocols, \PROTNAME{} does not try to mask neither type of failures in the round they occur.

In the case of benign failures, \PROTNAME{} settles for ensuring an all or nothing delivery semantics by relying on the WRB abstraction.
\iftoggle{FV}{
Recall from Section~\ref{sec:wrb} that WRB is implemented by running a OBBC instance on the message proposed in each round $r$.
Specifically, each node $p_i$ at round $r$ waits at most a given timeout $\delta_i^j$ for a message of the proposer $p_j$.
If it received the message, $p_i$ invokes the OBBC protocol and votes for delivering $p_j$'s message; otherwise, $p_i$ votes for skipping $p_j$'s message.
Yet, to avoid increasing the number of communication steps when the optimistic assumptions hold, we employ an OBBC protocol that terminates in a single step when all nodes propose the same value, e.g.,~\cite{Guerraoui2010} and Appendix~\ref{app:obbc}, and overlap the first step of the OBBC protocol of round $r$ with the proposal of round $r+1$.

A new block is decided on each communication step in which a single proposer broadcasts only its block and all others broadcast a single bit.
Further, if $p_i$ did not receive $p_j$'s message in round $r$, it increases $\delta_i^j$.
Hence, given the $\bDiamond \mathit{Sync}$ assumption, eventually each round started by a non-Byzantine proposer results in all nodes accepting its proposed block\footnote{In practice, for optimal performance we can dynamically adjust $\delta_i^j$ based on timing statistics gathered over some recency window.}.
}{
Recall from Section~\ref{sec:wrb} that WRB is implemented through an optimistic one round OBBC protocol that can piggyback another message on its initial vote broadcast.
Thus practically, the proposer of round $r+1$ piggybacks its proposed block on its vote for round $r$, obtaining the desired communication goals.
}

As for non-benign Byzantine failures, these may cause two correct nodes to initially accept two different block proposals in the same round $r$.
This is why initially we define a block to be only tentatively decided.
Due to the rotating proposer paradigm and the ratio between $f$ and $n$, if two different blocks are tentatively decided in a round $r$, then at worst by round $r+f$ there will be a round led by a correct proposer, who will report the same blockchain's authentication data to all nodes.
In that round nodes who discover that their blockchain history is different than the one reported by the proposer would initiate a \emph{recovery} phase in which a full fledged PBFT protocol~\cite{Castro1999} is invoked to decide on the longest possible blockchain given the transactions the nodes already know about.
Thus, the cost of the full fledged PBFT protocol is amortized among multiple blocks.

\begin{comment}
We first review how the algorithm preserves safety.
After establishing this basic idea, we will show a slight modification that handles liveness.

\paragraph{Handling safety:} We start by assuming that a node always delivers some message, but that the message might be different than messages delivered by other nodes due to Byzantine activity.
If every proposer is different from the last $f$ proposers, we know that in every $f+1$ rounds there is at least one correct proposer which, due to its correctness, sends an identical message to all.
Hence, by validating the authentication data that is associated with the new block, a correct node may possess a different version of the chain for at most $f$ rounds.
When contradicting versions are revealed, the nodes have to synchronized back into a single version.
\end{comment}

Given the above, it is clear that once a correct node reaches round $r+f+1$, it knows that the prefix of its blockchain upto round $r$ will never change, and therefore becomes definitely decided.
That is, \PROTNAME{} provides IPVC($f+1$).
Yet, to fulfill the IPVC($f+1$) properties, and for reasons that will be clarified in Section~\ref{sec:desc}, the recovery mechanism is based on the following invariant:
\begin{invariant}
	\label{inv:continue}
	A node $p$ proceeds to the next round of the algorithm only if it knows that at least $f+1$ correct nodes will eventually proceed as well.
\end{invariant}
An immediate consequence of Invariant~\ref{inv:continue} is that if a block $b^r$ is at depth $f+1$ in $p$'s local chain, then there are at least $f+1$ correct nodes for which $b^r$ is at depth of at least $f+1$ in their local chains.
%Preserving Invariant~\ref{inv:continue} ensures that while synchronized, every node delivers at least one version that contains the block of contention.
%We discuss the recovery method in details in Section~\ref{sec:desc}.
In principle, preserving Invariant~\ref{inv:continue} requires waiting to verify that at least $f$ other correct nodes are moving to the next round.
Yet, since the communication pattern we described above already includes an all-to-all message exchange in each round (while executing OBBC), it serves as an implicit acknowledgement, so we have a single message per round when the optimistic assumptions hold.

\begin{comment}
In exchange, for the sake of safety it has to postpone a decision for more $f + 1$  rounds\footnote{
One might think that a delay of $f$ rounds should be sufficient.
Alas, due to the asynchronous nature of the model, the protocol has to delay the permanent decision for one more round.
For more details see Theorem~\ref{thm4}.}.
\end{comment}

\begin{comment}
\paragraph{Handling liveness:} The logical jump from the presented solution to the full one is short: replace the progress message with a speculative BBC.
The nodes not only report their progress but also vote whether to deliver the proposer's message at all, e.g., due to a benign fault where some nodes received the message and some did not.
As most of the time the fault-free and synchronized case hold, the speculative BBC is expected to be terminated in a single communication step.
It is easy to fast terminate any type of consensus where there is no contention, although that in the multi-value case this is not a trivial requirement.
Here we circumvent the problem by performing consensus to agree on liveness rather than safety, resulting in that it is most likely that the nodes will vote the same.
\end{comment}

\begin{comment}
\paragraph{Normal Case Operation}
Figure~\ref{fig:nco} depicts a normal case operation for $n=4$ and $f=1$ where the system is in a synchronized period and no failures occur.
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{figures/normal.pdf}
\caption{The protocol under optimal conditions. The first round performs two communication steps. From then on, as long the optimistic conditions hold, the algorithm executes a single communication step for each new proposal.}
\label{fig:nco}
\end{figure}
In the normal case operation, a node $p_i$ performs one of the following actions in round $r$:
\begin{itemize}
\item If $p_i$ is the current proposer and round $r-1$ was not run under the optimistic conditions, then $p_i$ WRB-broadcasts a new signed proposal $v^r$ to all.
\item If $p_i$ is not the proposer of round $r+1$ and $p_i$ has received a proposal from $r$'s proposer, then $p_i$ broadcasts a \textsc{Vote} message.
The \textsc{Vote} message acts as the first BBC message.
\item If $p_i$ is the proposer of round $r+1$ and $p_i$ has received a proposal from $r$'s proposer, then $p_i$ broadcasts $v^{r+1}$, a new signed proposal, piggybacked to the required \textsc{Vote} message.
\end{itemize}
If BBC returned 1, then $p_i$ tentatively decides $v^r$ and definitely decides $v^{r-(f+2)}$.
In the normal case operation all nodes are expected to receive $v^r$ and to act correctly.
Hence, all nodes will broadcast \textsc{Vote}, terminating BBC in a single communication step while preserving Invariant~\ref{inv:continue}.
Finally, piggybacking $v^{r+1}$ on the \textsc{Vote} message yields a single communication step protocol.
\end{comment}

\subsection{Detailed Description}
\label{sec:desc}
\begin{algorithm}[t]
	\caption{\PROTNAME{} -- code for $p_i$}
	\label{alg1}
	\footnotesize
	\begin{algorithmic}[1]
		\State $r_i \leftarrow 0$
		\State $\mathit{proposer_{r_i}}\leftarrow p_0$
		\State $\mathit{full\_mode \leftarrow true}$
		\While {true}
		\State $b \leftarrow nil$
		\While {$\mathit{proposer_{r_i}}$'s block was tentatively decided in the last $f$ rounds} \label{alg1:lines:choose_a_proposer_b}
		\State $\mathit{proposer_{r_i}} \leftarrow (\mathit{proposer_{r_i}} + 1) \mod n$
		\EndWhile \label{alg1:lines:choose_a_proposer_e}
		\If {$i=\mathit{proposer_{r_i}} \land \mathit{full\_mode = true}$ } \Comment{executed if nil has been WRB-delivered in the last iteration} \label{alg1:lines:non-optimal-b} 
		\State $b \leftarrow$ prepared block
		\State \emph{WRB-broadcast(b)}
		\State $ b \leftarrow nil$
		\EndIf \label{alg1:lines:non-optimal-e}
		\If {$(\mathit{proposer_{r_i}} + 1) \mod{n} = i$} \label{alg1:lines:optimal-b}
		\State $b \leftarrow$ prepared block
	%	\State piggyback $(b)$ to the first message of \emph{WRB-deliver}
		\EndIf \label{alg1:lines:optimal-e}
		\State  $b_i^{r_i} \leftarrow$ \emph{WRB-deliver($\mathit{proposer_{r_i}}, b$)} \label{alg1:lines:deliver-b}
		\If {$b_i^{r_i} = nil$}
		\State $\mathit{full\_mode \leftarrow true}$
		\State $\mathit{proposer_{r_i}} \leftarrow (\mathit{proposer_{r_i}} + 1) \mod n$
		\State continue
		\EndIf \label{alg1:lines:deliver-e}
		\State $\mathit{full\_mode \leftarrow false}$
		\If {$b_i^{r_i} $ is not $valid$} \Comment {validating the block hash against the previous block} \label{alg1:lines:not-valid-b}
		\State {$proof\leftarrow (b_i^{r_i}, sig_{\mathit{proposer_{r_i}}}(b_i^{r_i}),\newline
			 b_i^{r_i-1}, sig_{\mathit{proposer_{r_i - 1}}}(b_i^{r_i-1}))$}
		\State \emph{RB-broadcast(proof)}
		\State invoke $RECOVERY(r_i, proof)$ \label{alg1:lines:not-valid-e}
		\State continue
		\EndIf
		\State append $b_i^{r_i}$ to the chain \label{alg1:lines:valid-b}
		\State decide $b_i^{r_i - (f + 2)}$
		\State $r_i \leftarrow r_i + 1$ \label{alg1:lines:valid-e}
		\EndWhile
		%	\State { }
		\\
		\State {$\text{\textbf{upon} \emph{RB-deliver} a valid }(b^{r}, sig_{\mathit{proposer_{r}}}(b^{r}),
			\newline b^{r-1}, sig_{\mathit{proposer_{r - 1}}}(b^{r-1}))\text{ \textbf{do}:}$} \label{alg1:lines:not-valid-received-b}
		\State {\indent invoke $RECOVERY(r, proof)$} \label{alg1:lines:not-valid-received-e}
        \\
		\Procedure {recovery}{r, proof}
		\State $\mathit{versions_r}\leftarrow \{\}$ 
		\If {$r_i < r - 1$} \label{alg1:lines:recovery:propose-b}
		\State $v \leftarrow \mathit{empty\_version}$
		\Else
		\State $v \leftarrow [(b^{r - (f + 1)}, sig_{\mathit{proposer_{r - (f + 1)}}}(b^{r - (f + 1)})), ...,
		\newline (b^{r - 1}, sig_{\mathit{proposer_{r - 1}}}(b^{r - 1})), ..., (b^{r_i}, sig_{\mathit{proposer_{r_i}}}(b^{r_i}))]$
		\EndIf
		\State \emph{Atomic-broadcast$(v)$} \label{alg1:lines:recovery:propose-e}
		\Repeat { \emph{Atomic-deliver} $v_j$ from $p_j$ } \label{alg1:lines:recovery:decide-b}
		\If {$v_j$ is $valid$} \Comment{validating the received version}
		\State $\mathit{versions_r} \leftarrow \mathit{versions_r} \cup \{v_j\}$
		\EndIf
		\Until {$|\mathit{versions_r}| = n - f$}
		\State $v' \leftarrow $ the first received among $\{v_j \in \mathit{versions_r} |r_j = max\{r_k | v_k \in \mathit{versions_r} \land (b^{r_k}, sig_{\mathit{proposer_{r_k}}}(b^{r_k}) \in v_k\} \}$
		\State adopt $v'$ and update $r_i$, and $\mathit{proposer_{r_i}}$ \label{alg1:lines:recovery:decide-e}
		\State $\mathit{full\_mode \leftarrow true}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

%\subsubsection{Description of the algorithm}
%\label{desc}

The pseudocode of \PROTNAME{} is listed in Algorithm~\ref{alg1}. % and~\ref{alg2}.
During each round $r$, $p_i$ takes the following actions:
\begin{itemize}
	\item First, $p_i$ identifies a proposer who did not successfully propose a block in the last $f+1$ rounds (lines~\ref{alg1:lines:choose_a_proposer_b}-\ref{alg1:lines:choose_a_proposer_e}).
	This is done using a deterministic rule, which guarantees that all correct nodes choose the same proposer.
	%Given the atomic order of \PROTNAME, it guarantees that all correct nodes choose the same proposer.
	\item Next, if $p_i$ is $r_i$'s proposer and $\mathit{full\_mode}=true$ (due to WRB-delivering $nil$ or returning from recovery),
	 %$\mathit{nil}$ has been WRB-delivered in the previous iteration (this includes the very first iteration),
	 then $p_i$ disseminates its block (lines~\ref{alg1:lines:non-optimal-b}-\ref{alg1:lines:non-optimal-e}). This part guarantees \PROTNAME's liveness if the previous piggybacked block has not been received by any correct node. 
	\item Similarly, if $p_i$ is supposed to be $(r_i + 1)$'s proposer, it prepares a block that is about to be piggybacked on the first message of \emph{WRB-deliver} (lines~\ref{alg1:lines:optimal-b}-\ref{alg1:lines:optimal-e}).
	\item Then, $p_i$ tries to \emph{WRB-deliver} the block from $r_i$'s proposer.
	If \emph{WRB-deliver} returns \emph{nil}, then $p_i$ continues to the next proposer and starts over  (lines~\ref{alg1:lines:deliver-b}-\ref{alg1:lines:deliver-e}).
	Else,\emph{WRB-deliver} returned a block $b_i^{r_i}$.
	\item If $b_i^{r_i}$ is valid, $p_i$ appends it to its chain and decides on the $(r_i - (f + 2))^{\mathrm{th}}$ block (lines~\ref{alg1:lines:valid-b}-\ref{alg1:lines:valid-e}).
	\item If $b_i^{r_i}$ is not valid, it means that some non-benign Byzantine activity has occurred.
	Hence, $p_i$ \emph{RB-broadcast} a proof that $b_i^{r_i}$ is invalid and invokes the recovery procedure (lines~\ref{alg1:lines:not-valid-b}-\ref{alg1:lines:not-valid-e}).
	\item Similarly, when $p_i$ \emph{RB-delivers} from $q$ a valid proof for $b_q^r$'s invalidity \iftoggle{FV}{(recall that validity is verified against the predefined \emph{valid} method and digital signatures),}{} it invokes the recovery procedure (lines~\ref{alg1:lines:not-valid-received-b}-\ref{alg1:lines:not-valid-received-e}).
\end{itemize}
The recovery procedure installs agreement among all correct nodes regarding the longest possible prefix of the blockchain.
Executing \textsc{RECOVERY} by $p_i$ involves:
\begin{itemize}
	\item $p_i$ proposes, using \emph{Atomic-broadcast}, a valid version of the $f$ blocks that are in disagreement (excluding $b^r$ itself) followed by all the newer blocks it knows about (lines~\ref{alg1:lines:recovery:propose-b}-\ref{alg1:lines:recovery:propose-e}).
	\item Then $p_i$ collects $n-f$ valid versions (including empty ones) and adopts the first longest agreed prefix of the blockchain (lines~\ref{alg1:lines:recovery:decide-b}-\ref{alg1:lines:recovery:decide-e}).
\end{itemize}
\iftoggle{FV}{
Notice that after executing the recovery protocol, nodes may rescind their round number to an earlier value.
Yet, due to asynchrony, some nodes might still be running in the pre-recovery version of these rounds.
Hence, it is important to distinguish between messages pertaining to be sent in the same round number where some of these messages were sent before a recovery while others were sent after the recovery (that rescinded the respective round).
To thet end, each execution of the recovery installs a new \emph{epoch} number and nodes are only willing to accept messages from their current or more advanced epochs.
To avoid obfuscation, the details are omitted from the code in Algorithm~\ref{alg1}.
}{
}

Given the algorithm's code and Invariant~\ref{inv:continue}, at any time there are at least $f+1$ correct nodes such that their current round is the most advanced.
We call this group the \emph{front} of the algorithm.
As $p_i$ waits until it receives $n-f$ valid versions, at least one of them has been proposed by $q \in \textit{front}$.
Following the \textbf{Atomic-Order} property all correct nodes will adopt the very same version.
Recall that a received version is valid if it satisfies the following:
\begin{enumerate}
	\item the digital signatures are correct,
	\item satisfies the predefined \textsc{valid} method and
	\item every $f+1$ consecutive blocks were created by $f+1$ different nodes.
\end{enumerate}
Thus, $f$ Byzantine nodes may propose a valid version in which the last $f$ blocks are switched by $f$ made up blocks that satisfy these three conditions.
Yet, as long as this version is valid with respect to the \textsc{valid} method, there is no need to preclude it~\cite{Luu:2016}.
%\textbf{[[[This whole last part is unclear.]]] {[\color{red} better?}]}

%\textbf{[[[Where is Invariant~\ref{inv:continue} being enforced?]]] {[\color{red} We wrote earlier that WRB implicit enforces it}]}

\iftoggle{FV}{
Figure~\ref{fig:nco} depicts a normal case operation for $n=4$ and $f=1$ where the system begins a synchronized period and no failures occur.
\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{figures/normal.pdf}
	\caption{\PROTNAME{} in the normal case operation.}
	\label{fig:nco}
\end{figure}
In this ``good period'', all nodes are expected to receive $b^r$ and to act correctly.
Hence, all nodes vote to receive $b^r$, terminating OBBC (and thus, by Observation~\ref{wrb:obs1}, WRB-deliver) in a single communication step while preserving Invariant~\ref{inv:continue}. 
In addition, piggybacking $b^{r+1}$ on $r$'s first WRB-deliver message ensures the desired communication goals.
The exception is the first round, in which no piggybacking may occur and therefore the first block (only) requires two communication steps.
}{}

\iftoggle{FV}{
\subsection{Correctness Proof}
\begin{lemma}[\emph{IVPC(f+1)-Validty}]
	\label{proof:lemma1}
	A decided (possible tentative) value $v$ satisfies the \textsc{valid} method.
\end{lemma}
\begin{proof}
	Following Algorithm~\ref{alg1}'s code, a value is appended to the blockchain only if it satisfies the \textsc{valid} method.
\end{proof}
\begin{lemma}
	\label{proof:lemma2}
	 Every $f+1$ consecutive decided blocks were proposed by $f+1$ different nodes.
\end{lemma}
\begin{proof}
	By Algorithm~\ref{alg1}'s code (lines 5-6), if the current proposer has successfully proposed a block in the last $f+1$ rounds, then its role is switched to a new proposer.
\end{proof}
\begin{lemma}
	\label{proof:lemma3}
	At the recovery procedure's end, all correct nodes adopt the same version.
\end{lemma}
\begin{proof}
	By the \textbf{Atomic-Order} of the atomic broadcast primitive all correct nodes receive the same versions in the same order. Hence, applying the deterministic rule described in Algorithm~\ref{alg1} results in an agreement among the correct nodes.
\end{proof}
\begin{lemma}
	\label{proof:lemma4}
	For any two correct nodes $p,q$, let $b_p^r, b_q^r$ be their decided value in round $r$.
	If $d(b_p^r) > f \wedge d(b_q^r) > f$ then $b_p^r=b_q^r$.
\end{lemma}
\begin{proof}
	Let $p,q$ be two correct nodes and let $b_p^r, b_q^r$ be their decided value in round $r$ such that $d(b_p^r) > f \wedge d(b_q^r) > f$ and assume b.w.o.c. that $b_p^r\neq b_q^r$.
	
Let $p_r$ be $r$'s proposer.
If $p_r$ is correct, then by \textbf{WRB-Agreement} and $p_r$'s correctness all correct nodes have received the very same message from $p_r$ (as in Reliable Broadcast).
Hence, the case of $b_p^r\neq b_q^r$ may occur only as a result of the recovery procedure invocation in round  $r' \in \{r+1, ..., r + f\}$.
By Lemma~\ref{proof:lemma3} at the end of the recovery procedure all correct nodes agree on the same version. Hence, $b_p^r = b_q^r$, contrary to the assumption.
	
Suppose that $p_r$ is Byzantine and has disseminated different blocks to $p$ and $q$.
Then, by Lemma~\ref{proof:lemma2} and the fact that the system model assumes at most $f$ faulty nodes there is at least one block $b^{r'} \in  \{b^{r+1}, ..., b^{r + f}\}$ that was proposed by correct proposer $p_{r'}$.
Due to $p_{r'}$'s correctness it disseminates the same block to all, including the associated authentication data.
Assume w.l.o.g. that $p_{r'}$ has received from $p_r$ the same version as $p$, then following Algorithm~\ref{alg1} (lines 19-22) $q$ receives an invalid block from $p_{r'}$ and invokes the recovery procedure.
As $q$ is correct and by \textbf{RB-Termination} $p$ RB-delivers $q$'s proof of $b_{q}^{r'}$ invalidity and triggers the recovery procedure.
Following Lemma~\ref{proof:lemma3} at the end of the recovery procedure all correct nodes adopt the very same version. Hence, $b_p^r = b_q^r$. A contradiction.
\end{proof}

\begin{lemma}[\emph{IVPC(f+1)-Agreement}]
	\label{proof:lemma5}
	For any two correct nodes $p,q$, let $b_p^r, b_q^r$ be their decided value in round $r$.
    If $d(b_p^r) > f+1 \wedge d(b_q^r) > f+1$ then $b_p^r=b_q^r$.
\end{lemma}
\begin{proof}
	Follows directly from Lemma \ref{proof:lemma4}.
\end{proof}

\begin{definition}
	\label{def:def1}
	Let $b_p^{r}, b_p^{r'}$ be two decided (possibly tentative) blocks of $p$ such that $r' > r$.
	$b_p^{r'}$ is \emph{valid with respect to} ${b_p^{r}}$ if the sub-chain $[b_p^r, b_p^{r+1}, ..., b_p^{r'}]$ satisfies the predefined \textsc{valid} method.
    Similarly, a sub-chain $[b_p^r, b_p^{r+1}, ..., b_p^{r'}]$ is \emph{valid with respect to} $b_p^{r - k}$, for some $ k \leq r$, if the sub-chain $[b_p^{r - k}, ..., b_p^{r}, ..., b_p^{r'}]$ satisfies the predefined \textsc{valid} method and each $f+1$ consecutive blocks are proposed by $f+1$ different proposers.
\end{definition}

\begin{lemma}
	\label{proof:lemma6}
	If during the recovery procedure for round $r$, a correct node $p$ receives a version $v$ from correct node $q$, then $v$ is valid with respect to $b_p^{r - (f + 2)}$.
\end{lemma}
\begin{proof}
	If the received version is an empty one, it is trivially valid with respect to $b_p^{r - (f + 2)}$.
	Else, by Lemma~\ref{proof:lemma4} all correct nodes agree on $b^{r -(f + 2)}$.
    As $q$ is correct, by Lemma \ref{proof:lemma1} $q$ appends only valid blocks to its blockchain.
    Hence, $q$'s version (that starts with $b_q^{r - (f + 1)}$) is valid with respect to $b_q^{r - (f + 2)}$ which is identical to $b_p^{r - (f + 2)}$.
\end{proof}
%\textbf{[[[Did we define what it means to be valid with respect to some block?]] {\color{red}better?}}

\begin{definition}
	\label{def:def2}
	Let $r_g$ be the most advanced round of the algorithm that any correct node runs.
    We define the group of nodes whose current round is $\in\{r_g, r_g -1\}$ by $\mathit{front}=\{p|r_p$ $\in \{r_g-1, r_g\}\}$.
    Note that as long as Invariant~\ref{inv:continue} is kept, there are at least $f+1$ correct nodes in \emph{front}.
\end{definition}

\begin{lemma}
	\label{proof:lemma7}
	As long as Invariant~\ref{inv:continue} is kept, a correct node executing the recovery procedure receives $n-f$ valid versions and at least one of them was received from a node in \emph{front}.
\end{lemma}
\begin{proof}
	By \textbf{RB-Termination} if a correct node $p$ detects an invalid block and invokes the recovery procedure, eventually every correct node will receive $p$'s proof and will invoke the recovery procedure.
	Following the system model, the ratio between $n$ and $f$ and Lemma~\ref{proof:lemma6}, a correct node does not get blocked while waiting for $n-f$ valid versions (part of whom may be empty). By Invariant~\ref{inv:continue}, $p$ receives at least one version from a correct node in $\mathit{front}$.
\end{proof}

\begin{lemma}[\emph{IVPC(f+1)-Termination(1)}]
	\label{proof:lemma8}
	Every round eventually terminates.
\end{lemma}
\begin{proof}
	Let $r$ be a round of the algorithm.
	As long WRB-deliver has returned $nil$, a correct proposer will propose its next block.
    Thus, by \emph{WRB-Termination(1)}, \emph{WRB-Termination(2)} and the algorithm's iterative nature every correct node eventually succeeds to \emph{WRB-deliver} $b^r \neq nil$.
    
    If $b^r$ is valid and the recovery procedure has not been invoked, then naturally nothing prevents the round from terminating.
    If the recovery procedure has been invoked, then following Lemma~\ref{proof:lemma7} every correct node eventually receives $n-f$ valid versions and finishes the recovery procedure; in the worst case, such a node stays in round $r-1$.
    The system model assumes at most $f$ faulty nodes, which means that the above can repeat itself at most $f$ times in a row.
    Hence, after at most $f$ consecutive invocations of the recovery procedure, a correct proposer proposes $b^r$, ensuring that $r$ terminates in all correct nodes.
\end{proof}
\begin{definition}
	\label{proof:def3}
	Let $r$ be a round of the algorithm, we define by $\textit{front}_r=\{p|r_p > r + f + 1\}$ the group of nodes whose current round is greater by at least $f+1$ rounds than $r$.
\end{definition}
\begin{lemma}[\emph{IVPC(f+1)-Termination(2}]
	\label{proof:lemma9}
	In every round $r' > r + f + 1$, $v_p^r$ is definite.
\end{lemma}
\begin{proof}
Following Algorithm~\ref{alg1}'s code, after a valid block is WRB-delivered, the only way it can be replaced is by an invocation of the recovery procedure.
By Algorithm~\ref{alg1}'s code and Lemma~\ref{proof:lemma7}, if the recovery procedure has been invoked regarding round $r$, then $p$ adopts a prefix version that was suggested by $q \in \textit{front}$.
Obviously, $\textit{front} \subseteq \textit{front}_r$. 
By Lemma~\ref{proof:lemma5}, $\forall q,p\in \textit{front}_r, b^r_q = b^r_p$.
In other words, $b^r_p$ is definite.

Note that the ratio between $n$ and $f$ as well as the version's validation test ensure that no Byzantine node is able to propose a version that does not include $b^r_q$. 
\end{proof}
Notice that due to asynchrony, it is possible that some node $q \in \mathit{front}$ advances to round $r+1$ while another node $p \in \mathit{front}$ invokes the recovery procedure for round $r+1$.
In such a case, $q$ may adopt a new blockchain prefix which was proposed by $p$ and thus replace $b_q^{r - (f+1)}$.
This edge case, illustrated in Figure~\ref{fig:edgecase}, is the reason why \PROTNAME{} implements \emph{IVPC(f+1)} rather than \emph{IVPC(f)}.
\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{figures/edge.pdf}
	\caption{If \PROTNAME{} would implement \emph{IVPC(f)} instead of \emph{IVPC(f+1)}, a node $q$ may renew a definite block.
		While recovering, due to contention on $b_q^r$, the nodes may adopt a prefix that was suggested by $p \in \mathit{front}$ while $p$ is still in round $r$.}
	\label{fig:edgecase}
\end{figure}

The following theorem follows from Lemmas~\ref{proof:lemma1}, \ref{proof:lemma5},~\ref{proof:lemma8} and~\ref{proof:lemma9}:
\begin{theorem}
	\label{proof:theorem1}
	The protocol listed in Algorithm~\ref{alg1} solves IVPC($f+1$).
\end{theorem}

\begin{lemma}[Atomic Order]
	\label{proof:lemma10}
		All blocks delivered by correct nodes using Algorithm~\ref{alg1} are delivered in the same order.
\end{lemma}
\begin{proof}
	Follows directly from Lemma~\ref{proof:lemma5} and the iterative nature of the algorithm.
\end{proof}

By Lemma~\ref{proof:lemma10} and Theorem~\ref{proof:theorem1}, we have:

\begin{theorem}
	The protocol listed in Algorithm~\ref{alg1} impose a total order of all blocks.
\end{theorem}

\begin{theorem}
	\label{thm:non-triv}
	The protocol listed in Algorithm~\ref{alg1} satisfies Non-Triviality.
\end{theorem}

The proof of Theorem~\ref{thm:non-triv} follows directly from Lemmas~\ref{proof:lemma8} and~\ref{proof:lemma9}, as well as the observation that correct nodes propose non-empty blocks whenever they hold clients' transactions that have not been included in any previously decided block.

}{
The correctness proof for Algorithm~\ref{alg1} is fairly technical. 
Due to space limitations, we defer it to the full version of this paper~\cite{BF2019full-anon}.
}

\begin{table}[t]
	\centering
	\begin{tabu} to 1\linewidth {||c|c|c|c||}
		\hline
		& \makecell{fault-\\free} & \makecell{Timing,\\and omission\\failures} &
		\makecell{Byzantine\\failures}\\
		\hline
		\hline
		\makecell{Communi-\\cation\\steps} & $1$ & $2+OBBC$ & \makecell{RB\\$+n$ parallel\\AB}\\
		\hline
		\makecell{Digital\\signature\\operations} & $1$ & $OBBC$ & \makecell{RB$+$AB\\$+(n -f)$\\$\cdot\text{(chain size)}$}\\
		\hline
		\makecell{Latency\\(in rounds)} & $f+1$ & \makecell{no additional\\overhead} & \makecell{no additional\\overhead}\\
		\hline
	\end{tabu}
	\caption{Performances characteristics of \PROTNAME. 
		RB and AB stand for Reliable and Atomic Broadcast respectively. 
		The first column shows the performance in the fault-free synchronized case. 
		The second column depicts the additional costs in an unsynchronized period and omission failures. 
		The third column depicts the additional expenses in the presence of a non-benign fault.}
	\label{performance:table1}
\end{table} 

\subsection{Theoretical Bounds and Performance}
\label{performance}
Table~\ref{performance:table1} summarizes the performance of \PROTNAME{} in each of its three modes.
In case of no failures and synchronized network, \PROTNAME{} performs in the OBBC of WRB-deliver a single all-to-all communication step as well as one digital signature operation.
Further, only one node broadcasts more than one bit.
This can be obtained since the latency for a definitive decision can be up to $f+1$ rounds.
%\iftoggle{FV}{We show in Section~\ref{sec:impl} that this tradeoff is quite reasonable.}{}
In case a message is not received by WRB-deliver due to timing, omission or benign failures, the algorithm runs the non optimistic phase of OBBC as well as two more communication steps (one-to-all and one-to-one) in which a node asks for the missed message from the nodes who did receive it.
Also, the amount of digital signature operations depends on the specific OBBC implementation that is used by WRB-deliver.
Finally, in case of Byzantine failures, \PROTNAME{} runs the recovery procedure which depends on the Reliable Broadcast and the Atomic Broadcast implementations.
\iftoggle{FV}{

Note that one can trade additional communication steps for fewer digital signature operations by using signature-free implementation of \PROTNAME's base protocols, e.g,~\cite{Mostfaoui:2015, Friedman:2005, Correia:2006}.
As \PROTNAME{} is inherently not signature-free, a node may authenticate up to $n-f$ received prefix versions.
}{}
Yet, when Byzantine failures manifest, a node does not lose blocks so the latency in terms of rounds remains the same.


==> sections/wrb.tex <==
\section{Weak Reliable Broadcast}
\label{sec:wrb}

\subsection{Overview}
\label{sec:wrb-overview}
We now present the \emph{Weak Reliable Broadcast} (WRB) abstraction which serves as \PROTNAME's main message dissemination mechanism.
WRB offers weaker agreement guarantees than \textbf{RB-Broadcast}~\cite{Bracha1987}.
In general, WRB ensures that the nodes agree on ($i)$ the sender's identity and ($ii$) whether to deliver a message at all, rather than the content of the message\footnote{
	To the best of our knowledge, we are the first to discuss WRB.
	Bracha's approach~\cite{Bracha1987} can be viewed as the opposite, first agree on the content of the message (\emph{consistent broadcast}), and then agree whether it should be delivered.}.
WRB is associated with the \emph{WRB-broadcast} and \emph{WRB-deliver} methods.
A node that wishes to disseminate a message $m$ invokes \emph{WRB-broadcast(m)}.
If a node expects to receive a message $m$ from $k$ through this mechanism it invokes \emph{WRB-deliver(k)}.
\emph{WRB-deliver(k)} returns a message $m$ where $m$ is the received message.
If the nodes were not able to deliver $k$'s message, \emph{WRB-deliver(k)} returns \emph{nil}.
Formally, WRB satisfies the following properties:
\iftoggle{FV}{
\iftoggle{MYACM}{
	\begin{description}
	}{	
		\begin{LaTeXdescription}
		}
	\item[WRB-Validity:] If a correct node \emph{WRB-delivered(k)} $m \neq nil$, then $k$ has invoked \emph{WRB-broadcast(m)}.
	\item[WRB-Agreement:] If two correct nodes $p,q$ \emph{WRB-delivered(k)} $m_p, m_q$ respectively from $k$, then either $m_p = m_q = nil$ or $m_p \neq nil \land m_q \neq nil$. 
	% Namely, all correct nodes either deliver a message different than $nil$ from $k$ or they all deliver $nil$.
	\item[WRB-Termination(1):] If a correct node $p$ \emph{WRB-deliver(k)} $m$ from $k$, then every correct node that is trying to \emph{WRB-deliver(k)} eventually \emph{WRB-deliver(k)} some message $m'$ from $k$.
	\item[WRB-Termination(2):] If a correct node $k$ repeatedly invokes \emph{WRB-broadcast(m)} then eventually all correct nodes will \emph{WRB-deliver(k)} $m$.
	\iftoggle{MYACM}{
\end{description}
}{	
\end{LaTeXdescription}
}
}{
\\
\noindent\textbf{*~WRB-Validity:} If a correct node \emph{WRB-delivered(k)} $m \neq nil$, then $k$ has invoked \emph{WRB-broadcast(m)}.\\
\noindent\textbf{*~WRB-Agreement:} If two correct nodes $p,q$ \emph{WRB-delivered(k)} $m_p, m_q$ respectively from $k$, then either $m_p = m_q = nil$ or $m_p \neq nil \land m_q \neq nil$.\\
%  Namely, all correct nodes either deliver a message different than $nil$ from $k$ or they all deliver $nil$.\\
\noindent\textbf{*~WRB-Termination(1):} If a correct node $p$ \emph{WRB-deliver(k)} $m$ from $k$, then every correct node that is trying to \emph{WRB-deliver(k)} eventually \emph{WRB-deliver(k)} some message $m'$ from $k$.\\
\noindent\textbf{*~WRB-Termination(2):} If a correct node $k$ repeatedly invokes \emph{WRB-broadcast(m)} then eventually all correct nodes will \emph{WRB-deliver(k)} $m$.
}

\subsection{Implementing WRB}
\label{sec:implWRB}
\begin{algorithm}[t]
	\caption{Weak Reliable Broadcast - code for $p$}
    \label{alg:wrb}
    \footnotesize
	\begin{algorithmic}[1]
		\State $\mathit{timer} \leftarrow \tau$ \label{alg:wrb:timer1}
		\Procedure{WRB-broadcast}{m}
		\State broadcast($m, \mathit{sig_p}(m)$) \Comment{push phase} \label{alg:wrb:broadcast}
		\EndProcedure
		\Procedure{WRB-deliver}{k} %, data}
		\State start $\mathit{timer}$ \Comment{$\mathit{timer}$'s value is set in either line \ref{alg:wrb:timer1} or in one of lines \ref{alg:wrb:deliver-increase-timer} \& \ref{alg:wrb:deliver-adjust-timer} of WRB-deliver's last invocation}
		\State \textbf{wait until} a valid $(m, \mathit{sig_k}(m))$ has been received or $\mathit{timer}$ has expired \label{alg:wrb:deliver-wait-until-timer}
		\If {a valid $(m, \mathit{sig_k}(m))$ has been received} 
		%\newline \Comment{$\mathit{sig_k}(m)$ has to be valid for the sake of lines \ref{alg:wrb:deliver-rec-req} - \ref{alg:wrb:deliver-rec-ans}} 
		\label{alg:wrb:deliver-message-received}
	%	\State $v \leftarrow 1 | data$
			\State $d \leftarrow \mathit{OBBC.propose}(1)$ 
			\Comment{If no node has proposed 0, then $\mathit{OBBC.propose}$ ends in a single communication step} \label{alg:wrb:deliver-vote-1}
		\Else
			\State $d \leftarrow \mathit{OBBC.propose(0)}$ \label{alg:wrb:deliver-vote-0}
	%	\State $v \leftarrow 0 | data$
		\EndIf
		\If {$d = 0$}  \label{alg:wrb:deliver-decided-0}
			\State increase $\mathit{timer}$ \label{alg:wrb:deliver-increase-timer}
			\State return $\mathit{nil}$ \label{alg:wrb:deliver-return-nil}
		\EndIf
	%	\State $d \leftarrow BBC.propose(v)$
		\If {a valid $(m, \mathit{sig_k}(m))$ has been received} \label{alg:wrb:deliver-decided-1}
	%	\State $timer \leftarrow timeout$
	        \State adjust $\mathit{timer}$ \label{alg:wrb:deliver-adjust-timer}
			\State return $m$ \label{alg:wrb:deliver-return-msg}
		\EndIf
	%	\State increase $\mathit{timer}$ \label{alg:wrb:deliver-increase-timer}
		
	%	\If{$d = 1$}  \label{alg:wrb:deliver-decided-1.2}
		%	\State $timer \leftarrow timeout$
		\State broadcast($\mathit{REQ}, k$) \Comment{pull phase} \label{alg:wrb:deliver-req}
	%	\ElsIf {$d = 0$}
		%\State $timer \leftarrow 2*timer$
	%	\State return $\mathit{nil}$ 
	%	\EndIf
		\State \textbf{wait until} a valid $(m', \mathit{sig_k}(m'))$ has been received \label{alg:wrb:deliver-wait-res}
		\State return $m'$ \label{alg:wrb:deliver-return-res}
		\\
		\State \textbf{upon} receiving $(\mathit{REQ}, k)$ from $q \land$ a valid $(m, \mathit{sig_k}(m))$ has been received \textbf{do}:  \label{alg:wrb:deliver-rec-req}
		\State {\indent send($m, \mathit{sig_k}(m)$)} to $q$  \label{alg:wrb:deliver-rec-ans}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

The pseudo-code implementation of WRB is listed in Algorithm~\ref{alg:wrb}.
To \emph{WRB-broadcast} a message, a node simply broadcasts it to everyone (line~\ref{alg:wrb:broadcast}).
When $p$ invokes \emph{WRB-deliver(k)} it performs the following:
\begin{itemize}
	\item It waits for at most $timer$ to receive $k$'s message (line~\ref{alg:wrb:deliver-wait-until-timer}).
	\item If such a valid message has been received, then $p$ votes to deliver it using an OBBC protocol.
			Else, $p$ votes against delivering $k$'s message (lines~\ref{alg:wrb:deliver-message-received}-\ref{alg:wrb:deliver-vote-0}).
			Recall that if no node has proposed 0, then OBBC ends in a single communication step.
	\item Assuming the decision is not to deliver (OBBC returned 0), $p$ returns $\mathit{nil}$ (lines~\ref{alg:wrb:deliver-decided-0}-\ref{alg:wrb:deliver-return-nil}).
	\item If it was decided to deliver the message (OBBC returned 1) and the message has already been received by $p$, $p$ returns it (lines~\ref{alg:wrb:deliver-decided-1}-\ref{alg:wrb:deliver-return-msg}).
	\item Else, since OBBC decided $1$, it means that at least one correct node was able to receive $k$'s message and voted for its acceptance. Thus, $p$ moves to a \emph{pull} phase and pulls $k$'s message from the nodes who did receive it.
	When $p$ eventually receives a valid message, $p$ returns it (lines~\ref{alg:wrb:deliver-req}-~\ref{alg:wrb:deliver-return-res}).
	\item Upon receiving $q$'s request for $k$'s message, if $p$ has $k$'s message $m$, it sends $(m, \mathit{sig_k}(m))$ back to $q$ (lines~\ref{alg:wrb:deliver-rec-req}-\ref{alg:wrb:deliver-rec-ans}).
	
%	\item On \iftoggle{FV}{obtaining}{} a valid response to $p$'s republish request, $p$ returns the received message (lines~\ref{alg:wrb:deliver-wait-res}-\ref{alg:wrb:deliver-return-res}).	 
\end{itemize}

To ensure liveness, the \emph{timer} is increased each time $p$ does not receive the message  (line~\ref{alg:wrb:deliver-increase-timer}).
To avoid having too long timers for too long, \emph{timer} is adjusted downward when a message is received by $p$ (line~\ref{alg:wrb:deliver-adjust-timer}).
The exact details of such adjustments are beyond the scope of this paper, but see for example~\cite{Castro1999}.

\iftoggle{FV}{
In a typical implementation of OBBC each node broadcasts its vote~\cite{obbc-paper,Raynal2018book}. % {\color{red} [which paper?]}~\cite{}.
Then if a node receives enough votes for the same value $v$ to safely decide $v$ after this single communication step, it decides $v$ and returns.
We present our own OBBC protocol in Appendix~\ref{app:obbc}.
}
{
In a typical implementation of OBBC each node broadcasts its vote~\cite{obbc-paper,Raynal2018book}. % {\color{red} [which paper?]}~\cite{}.
Then if a node receives enough votes for the same value $v$ to safely decide $v$ after this single communication step, it decides $v$ and returns.
We present our own OBBC protocol in the full version of this paper~\cite{BF2019full-anon}.
}
%[[{\color{red} considering the extra explanations on OBBC in the algorithm pseudo code and description, can we remove the above?}]]

\paragraph*{Piggybacking Over WRB-Deliver}
In order for \PROTNAME{} to maintain its amortized one communication step per block we need \PROTNAME{} to be able to piggyback one of its message types on another message it sends as part of the \emph{WRB-delivers} protocol.
The details appear in Section~\ref{sec:desc} below.
We support this by augmenting the \emph{WRB-deliver} method to receive two parameters, \emph{WRB-deliver(k,pgd)}, such that \emph{pgd} is the potential piggybacked data (can be $\mathit{nil}$).
The OBBC protocol is also augmented to receive \emph{pgd} and piggyback it on the first message it broadcasts.
Recall that we assume an OBBC protocol that always starts by having each node broadcast its vote.
Hence in the augmented protocol, each node that starts the OBBC protocol broadcasts its vote alongside the piggybacked \emph{pgd} message, which is made available to the calling code together with the decision value.

\iftoggle{FV}{
\subsection{WRB Correctness Proof}
\begin{lemma}[\emph{WRB-Validity}]
\label{lemma:wrb-validity}
	If a correct node $p$ \emph{WRB-delivered(k)} a message $m \neq nil$, then $k$ has invoked \emph{WRB-broadcast(m)}.
\end{lemma}

\begin{proof}
The system model assumes reliable channels.
Also, each node signs the messages it \emph{WRB-broadcasts}.
Hence, if a message $m$ is received and pass validation as being sent by $k$, then $k$ has indeed \emph{WRB-broadcast(m)}.
\end{proof}

\begin{lemma}[\emph{WRB-Agreement}]
\label{lemma:wrb-agreement}
If two correct nodes $p,q$ \emph{WRB-delivered(k)} $m_p, m_q$ respectively from $k$, then $m_p,m_q \neq nil$.
Namely, all correct nodes either deliver a message different than $nil$ from $k$ or they all deliver $nil$.
\end{lemma}

\begin{proof}
Let $p,q$ be two correct nodes that have \emph{WRB-delivered(k)} $m_p, m_q$ respectively from $k$.
Assume b.w.o.c and w.l.o.g that $m_p \neq nil$ while $m_q = nil$.
A correct node may return $nil$ only if \emph{OBBC.propose} returns $0$.
Respectively, a correct node returns $m\neq nil$ only if \emph{OBBC.propose} returned $1$.
This is in contradiction to \textbf{BBC-Agreement}.
Hence, either $m_p, m_q \neq nil$ or both $p$ and $q$ return $nil$.
\end{proof}

\begin{lemma}[\emph{WRB-Termination[1]}]
\label{lemma:wrb-termination1}
If a correct node $p$ \emph{WRB-deliver(k)} $m$ from $k$, then every correct node that is trying to \emph{WRB-deliver(k)} eventually \emph{WRB-deliver(k)} some message $m'$ from $k$.
\end{lemma}

\begin{proof}
A node $p$ waits for $k$'s message at most $timer$ time units.
Hence $p$ eventually invokes \emph{OBBC.propose}.
By \textbf{BBC-Termination}, no correct node is blocked forever on \emph{OBBC.propose}.
If \emph{OBBC.propose} has returned $0$ then $p$ returns $nil$.
Else, if $k$'s message has been received by $p$ it returns $m$.
Otherwise, $p$ asks from other nodes for $k$'s message.
By \textbf{BBC-Validity}, if \emph{OBBC.propose} returns a value $v$ then at least one correct node $q$ proposed $v$.
Thus, if \emph{OBBC.propose} returned $1$ it means that at least one correct node $q$ has proposed $1$ and by the algorithm's code $q$ does so if it has received $k$'s message $m$.
Hence, when $q$ receives $p$'s request it sends back $m$.
As $q$ is correct $p$ receives and returns~$m$.
\end{proof}

\begin{lemma}[\emph{WRB-Termination[2]}]
\label{lemma:wrb-termination2}
If a correct node $k$ repeatedly invokes \emph{WRB-broadcast(m)} then eventually all correct nodes will \emph{WRB-deliver(k)} $m$.
\end{lemma}

\begin{proof}
By the algorithm's code, on any unsuccessful delivery the timer increases.
Let $k$ be a correct node that repeatedly invokes \emph{WRB-broadcast(m)}.
Following the $\bDiamond Synch$ \cite{Bouzid2015} assumption and the incremental timer method \cite{Castro1999}, eventually after an unknown time $\tau$ the timer of all nodes is longer than the unknown upper bound $\delta$ on a message's transfer delay.
Hence, every correct node receives $k$'s message and invokes \emph{OBBC.propose(1)}.
By \textbf{BBC-Agreement} if all correct nodes propose $1$ then $1$ has to be decided.
Hence, every correct node eventually \emph{WRB-deliver(k)} $m$.
\end{proof}

By the above four lemmas we have:
\begin{theorem}
The protocol listed in Algorithm~\ref{alg:wrb} solves WRB.
\end{theorem}

\begin{observation}
	\label{wrb:obs1}
	If for every node OBBC decides in a single communication step, then WRB-deliver also terminates in a single communication step.
\end{observation}
}
{
Since the correctness proof of Algorithm~\ref{alg:wrb} is technical, it is deferred to the full version of this paper~\cite{BF2019full-anon}.
}

